Comparative Study of Eight Formal Specifications of the Message Authenticator Algorithm

The Message Authenticator Algorithm (MAA) is one of the first cryptographic functions for computing a Message Authentication Code. Between 1987 and 2001, the MAA was adopted in international standards (ISO 8730 and ISO 8731-2) to ensure the authenticity and integrity of banking transactions. In 1990 and 1991, three formal, yet non-executable, specifications of the MAA (in VDM, Z, and LOTOS) were developed at NPL. Since then, five formal executable specifications of the MAA (in LOTOS, LNT, and term rewrite systems) have been designed at INRIA Grenoble. This article provides an overview of the MAA and compares its formal specifications with respect to common-sense criteria, such as conciseness, readability, and efficiency of code generation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{41}
\providecommand{\publicationstatus}{John P. Gallagher, Rob van Glabbeek and Wendelin Serwe (Eds):\\
Models for Formal Analysis of Real Systems (MARS'18)\\
and Verification and Program Transformation (VPT'18)
\\
EPTCS 268, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.268.2}{10.4204/EPTCS.268.2}}

